Multi-Task Meta Learning: learn how to adapt to unseen tasks

This work proposes Multi-task Meta Learning (MTML), integrating two learning paradigms Multi-Task Learning (MTL) and meta learning, to bring together the best of both worlds. In particular, it focuses simultaneous learning of multiple tasks, an element of MTL and promptly adapting to new tasks, a quality of meta learning. It is important to highlight that we focus on heterogeneous tasks, which are of distinct kind, in contrast to typically considered homogeneous tasks (e.g., if all tasks are classification or if all tasks are regression tasks). The fundamental idea is to train a multi-task model, such that when an unseen task is introduced, it can learn in fewer steps whilst offering a performance at least as good as conventional single task learning on the new task or inclusion within the MTL. By conducting various experiments, we demonstrate this paradigm on two datasets and four tasks: NYU-v2 and the taskonomy dataset for which we perform semantic segmentation, depth estimation, surface normal estimation, and edge detection. MTML achieves state-of-the-art results for three out of four tasks for the NYU-v2 dataset and two out of four for the taskonomy dataset. In the taskonomy dataset, it was discovered that many pseudo-labeled segmentation masks lacked classes that were expected to be present in the ground truth; however, our MTML approach was found to be effective in detecting these missing classes, delivering good qualitative results. While, quantitatively its performance was affected due to the presence of incorrect ground truth labels. The the source code for reproducibility can be found at https://github.com/ricupa/MTML-learn-how-to-adapt-to-unseen-tasks.

==> fig_matrix/matrix.tex <==
\begin{figure*}[ht]
\vspace{-0.3cm}
\begin{center}
\begin{tabular}{c c c c c | c c c c}
% \toprule
\footnotesize{Dataset} &  \multicolumn{4}{c}{\footnotesize{Taskonomy}} &  \multicolumn{4}{c}{\footnotesize{NYU}}\\
% & & & & \\
\footnotesize{Image} &  \multicolumn{4}{c}{\adjustimage{height=1.5cm,valign=m}{images/taskonomy/image.jpg}} & \multicolumn{4}{c}{\adjustimage{height=1.5cm,valign=m}{images/NYU/image.png}}\\
% & & & & \\
Tasks & Seg. & Depth & SN & Edge & Seg. & Depth & SN & Edge\\
% & & & & \\
\footnotesize{Ground Truth} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy/mask_seg.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy/mask_depth.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy/mask_surface.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy/mask_edge.jpg} & \adjustimage{height=1.5cm,valign=m}{images/NYU/mask_seg.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU/mask_depth.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU/mask_surface.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU/mask_edge.png}\\
% & & & & \\
\footnotesize{Single task} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy/single_seg.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy/single_depth.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy/single_surface.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy/single_edge.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU/single_seg.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU/single_depth.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU/single_surface.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU/single_edge.jpg}\\
% & & & & \\
\footnotesize{\ac{MTL}} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy/multi_seg.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy/multi_depth.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy/multi_surface.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy/multi_edge.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU/multi_seg.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU/multi_depth.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU/multi_surface.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU/multi_edge.jpg}\\
% & & & & \\
\footnotesize{\ac{MTML}} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy/meta_multi_seg.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy/meta_multi_depth.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy/meta_multi_surface.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy/meta_multi_edge.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU/meta_multi_seg.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU/meta_multi_depth.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU/meta_multi_surface.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU/meta_multi_edge.jpg}
\end{tabular}
\end{center}
\vspace{-0.45cm}
\caption{The figure illustrates sample images of the input, its corresponding ground truths, single task (Exp. 1), \ac{MTL} (Exp. 2.3) and \ac{MTML} (Exp. 5.4) outputs for semantic segmentation (Seg.), depth estimation (Depth), surface normal estimation (SN), and edge detection (Edge) for both the NYU-v2 and taskonomy datasets. Note: single-task models were trained individually for all tasks, while \ac{MTL} and \ac{MTML} used a multi-task network architecture.} 
\vspace{-0.45cm}
\label{fig:img_mat}
\end{figure*}

==> fig_matrix/seg_only.tex <==
\begin{figure*}[ht]
\subfloat[][Image]{\includegraphics[width=2.95cm]{images/seg_img_supp/box.jpg}}~
\subfloat[][GT]{\includegraphics[width=3cm]{images/seg_img_supp/segmask_box.jpg}}~
\subfloat[][Prediction]{\includegraphics[width=3cm]{images/seg_img_supp/seg_output_box.jpg}} ~
\subfloat[][Activation map: Vase]{\includegraphics[width=3cm]{images/seg_img_supp/act_map.png}} 
\end{figure*}

\begin{figure*}[ht]
\subfloat[][Image]{\includegraphics[width=2.95cm]{images/seg_img_supp/box1.jpg}}~
\subfloat[][GT]{\includegraphics[width=3cm]{images/seg_img_supp/segmask_box1.jpg}}~
\subfloat[][Prediction]{\includegraphics[width=3cm]{images/seg_img_supp/seg_output_box1.jpg}} ~
\subfloat[][Activation map : potted plant]{\includegraphics[width=3cm]{images/seg_img_supp/act_map1.png}} 
\end{figure*}

\begin{figure*}[ht]
\subfloat[][Image]{\includegraphics[width=2.95cm]{images/seg_img_supp/box4.jpg}}~
\subfloat[][GT]{\includegraphics[width=3cm]{images/seg_img_supp/segmask_box4.jpg}}~
\subfloat[][Prediction]{\includegraphics[width=3cm]{images/seg_img_supp/seg_output_box4.jpg}} ~
\subfloat[][Activation map: TV]{\includegraphics[width=3cm]{images/seg_img_supp/act_map4.png}} 
\end{figure*}
\begin{figure*}[ht]
\subfloat[][Image]{\includegraphics[width=2.95cm]{images/seg_img_supp/box5.jpg}}~
\subfloat[][GT]{\includegraphics[width=3cm]{images/seg_img_supp/segmask_box5.jpg}}~
\subfloat[][Prediction]{\includegraphics[width=3cm]{images/seg_img_supp/seg_output_box5.jpg}} ~
\subfloat[][Activation map: chair]{\includegraphics[width=3cm]{images/seg_img_supp/act_map5_chair.png}} ~
\subfloat[][Activation map: couch]{\includegraphics[width=3cm]{images/seg_img_supp/act_map5_couch.png}} 
\end{figure*}
\begin{figure*}[ht]
\subfloat[][Image]{\includegraphics[width=2.95cm]{images/seg_img_supp/box6.jpg}}~
\subfloat[][GT]{\includegraphics[width=3cm]{images/seg_img_supp/segmask_box6.jpg}}~
\subfloat[][Prediction]{\includegraphics[width=3cm]{images/seg_img_supp/seg_output_box6.jpg}} ~
\subfloat[][Activation map: chair]{\includegraphics[width=3cm]{images/seg_img_supp/act_map6.png}} 

\caption{This figure shows (a) the input RGB image, (b) the corresponding ground truth (GT) segmentation mask, and (c) the predicted segmentation mask (Prediction) by the \ac{MTML} model. The red box highlights the object not present in the ground truth (pseudo labels), but the proposed \ac{MTML} model learns to detect and segment them. (d) and (e) shows the class activation map for the missing or wrong classes.}
%Same with the sofa in the image (d), which is segmented in the predicted output but not in the given segmentation mask.}
\label{supp_seg_only}
\end{figure*}

==> fig_matrix/supp_matrix.tex <==
% \usepackage{multirow}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.5}
\begin{figure*}[ht]
\begin{center}

\begin{tabular}{c c c c c c| c c c c c}
\hline
\multirow[b]{ 2}{*}{\rotatebox[origin=t]{90}{Models}} & Input &  \multicolumn{4}{c}{\textbf{Taskonomy}} & Input & \multicolumn{4}{c}{\textbf{NYU}}\\ \cmidrule(lr){3-6} \cmidrule(lr){8-11}
% & & & & \\
& Image & Seg. & Depth & SN & Edge & Image & Seg. & Depth & SN & Edge\\
\hline
% \footnotesize{Image} &  \multicolumn{4}{c}{\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f8/image.jpg}} & \multicolumn{4}{c}{\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/image.png}}\\
% & & & & \\

% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{GT}} & \multirow[b]{ 4}{*}{\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f8/image.jpg}} &
\adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f8/segmask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f8/depthmask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f8/surface_normal_mask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f8/edge_mask.jpg} &
\multirow[b]{ 4}{*}{\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/image.png}}&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/segmask.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/depthmask.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/surface_normal_mask.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/edge_mask.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{Single}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f8/single_seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f8/single_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f8/single_surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f8/single_edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/single_seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/single_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/single_surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/single_edge_output.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{\ac{MTL}}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f8/multi_seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f8/multi_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f8/multi_surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f8/multi_edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/multi_seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/multi_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/multi_surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/multi_edge_output.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{\ac{MTML}}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f8/seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f8/depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f8/surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f8/edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/edge_output.png}\\

\hline
\footnotesize{\rotatebox[origin=c]{90}{GT}} & \multirow[b]{ 4}{*}{\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f9/image.jpg}} &
\adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f9/segmask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f9/depthmask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f9/surface_normal_mask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f9/edge_mask.jpg} &
\multirow[b]{ 4}{*}{\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/image.png}}&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/segmask.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/depthmask.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/surface_normal_mask.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/edge_mask.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{Single}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f9/single_seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f9/single_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f9/single_surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f9/single_edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/single_seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/single_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/single_surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/single_edge_output.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{\ac{MTL}}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f9/multi_seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f9/multi_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f9/multi_surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f9/multi_edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/multi_seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/multi_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/multi_surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/multi_edge_output.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{\ac{MTML}}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f9/seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f9/depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f9/surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f9/edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f2/edge_output.png}\\

\hline
\footnotesize{\rotatebox[origin=c]{90}{GT}} & \multirow[b]{ 4}{*}{\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f10/image.jpg}} &
\adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f10/segmask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f10/depthmask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f10/surface_normal_mask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f10/edge_mask.jpg} &
\multirow[b]{ 4}{*}{\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/image.png}}&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/segmask.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/depthmask.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/surface_normal_mask.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/edge_mask.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{Single}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f10/single_seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f10/single_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f10/single_surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f10/single_edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/single_seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/single_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/single_surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/single_edge_output.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{\ac{MTL}}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f10/multi_seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f10/multi_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f10/multi_surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f10/multi_edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/multi_seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/multi_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/multi_surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/multi_edge_output.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{\ac{MTML}}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f10/seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f10/depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f10/surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f10/edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f3/edge_output.png}\\


% % & & & & \\

\end{tabular}
    
\end{center}
% \vspace{-0.45cm}
% \caption{The figure illustrates sample images of the input, its corresponding ground truths, single task (Exp. 1), \ac{MTL} (Exp. 2.3) and \ac{MTML} (Exp. 5.4) outputs for semantic segmentation (Seg.), depth estimation (Depth), surface normal estimation (SN), and edge detection (Edge) for both the NYU-v2 and taskonomy_mat datasets. Note: single-task models were trained individually for all tasks, while \ac{MTL} and \ac{MTML} used a multi-task network architecture.} 

\label{fig:img_mat_1}
\end{figure*}


\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.5}
\begin{figure*}[ht]
\begin{center}

\begin{tabular}{c c c c c c| c c c c c}
\hline
\multirow[b]{ 2}{*}{\rotatebox[origin=t]{90}{Models}} & Input &  \multicolumn{4}{c}{\textbf{Taskonomy}} & Input & \multicolumn{4}{c}{\textbf{NYU}}\\ \cmidrule(lr){3-6} \cmidrule(lr){8-11}
% & & & & \\
& Image & Seg. & Depth & SN & Edge & Image & Seg. & Depth & SN & Edge\\
\hline
% \footnotesize{Image} &  \multicolumn{4}{c}{\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f8/image.jpg}} & \multicolumn{4}{c}{\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f1/image.png}}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{GT}} & \multirow[b]{ 4}{*}{\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f15/image.jpg}} &
\adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f15/segmask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f15/depthmask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f15/surface_normal_mask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f15/edge_mask.jpg} &
\multirow[b]{ 4}{*}{\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/image.png}}&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/segmask.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/depthmask.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/surface_normal_mask.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/edge_mask.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{Single}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f15/single_seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f15/single_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f15/single_surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f15/single_edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/single_seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/single_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/single_surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/single_edge_output.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{\ac{MTL}}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f15/multi_seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f15/multi_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f15/multi_surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f15/multi_edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/multi_seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/multi_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/multi_surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/multi_edge_output.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{\ac{MTML}}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f15/seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f15/depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f15/surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f15/edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f9/edge_output.png}\\

\hline

\footnotesize{\rotatebox[origin=c]{90}{GT}} & \multirow[b]{ 4}{*}{\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f16/image.jpg}} &
\adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f16/segmask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f16/depthmask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f16/surface_normal_mask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f16/edge_mask.jpg} &
\multirow[b]{ 4}{*}{\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/image.png}}&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/segmask.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/depthmask.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/surface_normal_mask.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/edge_mask.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{Single}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f16/single_seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f16/single_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f16/single_surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f16/single_edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/single_seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/single_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/single_surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/single_edge_output.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{\ac{MTL}}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f16/multi_seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f16/multi_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f16/multi_surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f16/multi_edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/multi_seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/multi_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/multi_surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/multi_edge_output.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{\ac{MTML}}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f16/seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f16/depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f16/surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f16/edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f6/edge_output.png}\\

\hline
\footnotesize{\rotatebox[origin=c]{90}{GT}} & \multirow[b]{ 4}{*}{\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f17/image.jpg}} &
\adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f17/segmask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f17/depthmask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f17/surface_normal_mask.jpg} & \adjustimage{height=1.46cm,valign=m}{images/taskonomy_mat/f17/edge_mask.jpg} &
\multirow[b]{ 4}{*}{\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/image.png}}&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/segmask.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/depthmask.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/surface_normal_mask.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/edge_mask.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{Single}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f17/single_seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f17/single_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f17/single_surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f17/single_edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/single_seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/single_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/single_surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/single_edge_output.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{\ac{MTL}}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f17/multi_seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f17/multi_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f17/multi_surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f17/multi_edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/multi_seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/multi_depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/multi_surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/multi_edge_output.png}\\
% & & & & \\
\footnotesize{\rotatebox[origin=c]{90}{\ac{MTML}}} & &
\adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f17/seg_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f17/depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f17/surface_output.png} & \adjustimage{height=1.5cm,valign=m}{images/taskonomy_mat/f17/edge_output.png} &
&
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/seg_output.png} & 
\adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/depth_output.png} & \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/surface_output.png}& \adjustimage{height=1.5cm,valign=m}{images/NYU_mat/f8/edge_output.png}\\


\end{tabular}
    
\end{center}
% \vspace{-0.45cm}
\caption{The figure illustrates images of the input, its corresponding ground truths, single task (Exp. 1), \ac{MTL} (Exp. 2.3) and \ac{MTML} (Exp. 5.4) outputs for semantic segmentation (Seg.), depth estimation (Depth), surface normal estimation (SN), and edge detection (Edge) for both the NYU-v2 and taskonomy datasets. Note: single-task models were trained individually for all tasks, while \ac{MTL} and \ac{MTML} used a multi-task network architecture.} 

\label{fig:img_mat_supp}
\end{figure*}

==> fig_matrix/temp.tex <==
\subfloat[][Image]{\includegraphics[width=2.95cm]{images/seg_img_supp/box.jpg}}~
\subfloat[][GT]{\includegraphics[width=3cm]{images/seg_img_supp/segmask_box.jpg}}~
\subfloat[][Prediction]{\includegraphics[width=3cm]{images/seg_img_supp/seg_output_box.jpg}} ~
\subfloat[][Activation map: Vase]{\includegraphics[width=3cm]{images/seg_img_supp/act_map.png}} 
\\
\subfloat[][Image]{\includegraphics[width=2.95cm]{images/seg_img_supp/box1.jpg}}~
\subfloat[][GT]{\includegraphics[width=3cm]{images/seg_img_supp/segmask_box1.jpg}}~
\subfloat[][Prediction]{\includegraphics[width=3cm]{images/seg_img_supp/seg_output_box1.jpg}} ~
\subfloat[][Activation map : potted plant]{\includegraphics[width=3cm]{images/seg_img_supp/act_map1.png}} 
\\
\subfloat[][Image]{\includegraphics[width=2.95cm]{images/seg_img_supp/box4.jpg}}~
\subfloat[][GT]{\includegraphics[width=3cm]{images/seg_img_supp/segmask_box4.jpg}}~
\subfloat[][Prediction]{\includegraphics[width=3cm]{images/seg_img_supp/seg_output_box4.jpg}} ~
\subfloat[][Activation map: TV]{\includegraphics[width=3cm]{images/seg_img_supp/act_map4.png}} 
\\
\subfloat[][Image]{\includegraphics[width=2.95cm]{images/seg_img_supp/box5.jpg}}~
\subfloat[][GT]{\includegraphics[width=3cm]{images/seg_img_supp/segmask_box5.jpg}}~
\subfloat[][Prediction]{\includegraphics[width=3cm]{images/seg_img_supp/seg_output_box5.jpg}} ~
\subfloat[][Activation map: chair]{\includegraphics[width=3cm]{images/seg_img_supp/act_map5_chair.png}} ~
\subfloat[][Activation map: couch]{\includegraphics[width=3cm]{images/seg_img_supp/act_map5_couch.png}} 
\\
\subfloat[][Image]{\includegraphics[width=2.95cm]{images/seg_img_supp/box6.jpg}}~
\subfloat[][GT]{\includegraphics[width=3cm]{images/seg_img_supp/segmask_box6.jpg}}~
\subfloat[][Prediction]{\includegraphics[width=3cm]{images/seg_img_supp/seg_output_box6.jpg}} ~
\subfloat[][Activation map: chair]{\includegraphics[width=3cm]{images/seg_img_supp/act_map6.png}} 

==> tables/epoch_NYU.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[ht]
\centering

\caption{Table expressing the average number of training epochs for all the experiments for the NYU dataset.}
\label{tab:epochs_NYU}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lllcccc}
\hline
\textbf{Exp. No.} & \multicolumn{2}{c}{\textbf{Tasks Involved}} & \multicolumn{4}{c}{\textbf{Tasks}} \\ \hline
\textbf{} & \multicolumn{1}{c}{\textbf{Trained}} & \multicolumn{1}{c}{\textbf{Tested}} & \textbf{T1} & \textbf{T2} & \textbf{T3} & \textbf{T4} \\ \hline
 &  & \multicolumn{1}{c}{( also new tasks} & \textbf{Segmentation} & \textbf{Depth Estimation} & \textbf{Surface Normal} & \textbf{Edge Detection} \\
 &  & \multicolumn{1}{c}{added)} &  &  &  &  \\ \hline
\textbf{1} & \multicolumn{6}{c}{\textbf{Single task learning}} \\ \hline
 &  &  & 135 & 115 & 159 & 440 \\ \hline
\textbf{2} & \multicolumn{6}{c}{\textbf{Multi-task learning}} \\ \hline
2.1 & T1, T2 & T1, T2 & 125 & 125 & - & - \\
2.2 & T1, T2, T3 & T1, T2, T3 & 139 & 119 & 126 & - \\
2.3 & T1, T2, T3, T4 & T1, T2, T3, T4 & 156 & 136 & 141 & 156 \\
 &  &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\textbf{3} & \multicolumn{6}{c}{\textbf{Multi-task learning, addition of new task}} \\ \hline
3.1 & T1, T2 & T1, T2 (+ T3) & 126+49 & 126+0 & 58 &  \\
3.2 & T1, T2 & T1, T2 (+ T3, T4) & 126+49 & 126+22 & 93 & 160 \\
3.3 & T1, T2, T3 & T1, T2, T3 (+T4) & 140+49 & 119+0 & 127+42 & 60 \\ \hline
\textbf{4} & \multicolumn{6}{c}{\textbf{Multi-task learning, addition of new task with 50\% less training data}} \\ \hline
4.1 & T1, T2 & T1, T2 (+ T3) & 126+75 & 126+24 & 65 &  \\
4.2 & T1, T2 & T1, T2 (+ T3, T4) & 126+75 & 126+23 & 109 & 129 \\
4.3 & T1, T2, T3 & T1, T2, T3 (+T4) & 140+38 & 119+17 & 127+6 & 229 \\ \hline
\textbf{5} & \multicolumn{6}{c}{\textbf{Meta multi-task learning, meta testing phase involves addition of new task}} \\ \hline
5.1 & T1, T2 & T1, T2 (+ T3) & 422+20 & 334 & 48 & - \\
5.2 & T1, T2 & T1, T2 (+ T3, T4) & 422+13 & 334+0 & 38 & 40 \\
5.3 & T1, T2, T3 & T1, T2, T3 (+T4) & 357+18 & 285+16 & 358+9 & 58 \\
5.4 & T1, T2, T3, T4 & T1, T2, T3, T4 & 355 & 405 & 448 & 23 \\ \hline
\textbf{6} & \multicolumn{6}{c}{\textbf{Meta multi-task learning, meta testing phase involves addition of new task; with 50\% training data of new task}} \\ \hline
6.1 & T1, T2 & T1, T2 (+ T3) & 422+40 & 334 & 45 & -  \\
6.2 & T1, T2 & T1, T2 (+ T3, T4) & 422+22 & 334 & 56 & 64 \\
6.3 & T1, T2, T3 & T1, T2, T3 (+T4) & 398+43 & 255+1 & 399+17 & 54 \\ \hline
\textbf{7} & \multicolumn{6}{c}{\textbf{Multi-task learning, leave one task out format}} \\ \hline
7.1 & T2, T3, T4 & T2, T3, T4 & - & 90 & 99 & 161 \\
7.2 & T1, T3, T4 & T1, T3, T4 & 121 & - & 87 & 442 \\
7.3 & T1, T2, T4 & T1, T2, T4 & 131 & 111 & - & 438 \\
7.4 & T1, T2, T3 & T1, T2, T3 & 139 & 119 & 126 & - \\ \hline
\textbf{8} & \multicolumn{6}{c}{\textbf{Multi-task learning, leave one task out format, addition of the left out task}} \\ \hline
8.1 & T2, T3, T4 & T2, T3, T4 (+ T1) & 100 & 90+34 & 100+34 & 162+65 \\
8.2 & T1, T3, T4 & T1, T3, T4 (+T2) & 121+49 & 40 & 87+34 & 442+1 \\
8.3 & T1, T2, T4 & T1, T2, T4 (+T3) & 131+38 & 111+52 & 53 & 422+72 \\
8.4 & T1, T2, T3 & T1, T2, T3 (+T4) & 140+49 & 119 & 127+42 & 60 \\ \hline
\textbf{9} & \multicolumn{6}{c}{\textbf{Meta multi-task learning, leave one task out format, addition of left out task in meta testing}} \\ \hline
9.1 & T2, T3, T4 & T2, T3, T4 (+ T1) & 36 & 318+3 & 396+6 & 392+6 \\
9.2 & T1, T3, T4 & T1, T3, T4 (+T2) & 224+21 & 58 & 279+7 & 302+6 \\
9.3 & T1, T2, T4 & T1, T2, T4 (+T3) & 372+52 & 386+31 & 51 & 455+10 \\
9.4 & T1, T2, T3 & T1, T2, T3 (+T4) & 363+18 & 285+26 & 364+6 & 54 \\ \hline
\end{tabular}%
}
\end{table*}

==> tables/epoch_taskonomy.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[ht]
\centering
\caption{Table expressing the average number of training epochs for all the experiments for the taskonomy dataset.}
\label{tab:epochs_taskonomy}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lllcccc}
\hline
\textbf{Exp. No.} & \multicolumn{2}{c}{\textbf{Tasks Involved}} & \multicolumn{4}{c}{\textbf{Tasks}} \\ \hline
\textbf{} & \multicolumn{1}{c}{\textbf{Trained}} & \multicolumn{1}{c}{\textbf{Tested}} & \textbf{T1} & \textbf{T2} & \textbf{T3} & \textbf{T4} \\ \hline
 &  & \multicolumn{1}{c}{( also new tasks} & \textbf{Segmentation} & \textbf{Depth Estimation} & \textbf{Surface Normal} & \textbf{Edge Detection} \\
 &  & \multicolumn{1}{c}{added)} &  &  &  &  \\ \hline
\textbf{1} & \multicolumn{6}{c}{\textbf{Single task learning}} \\ \hline
 &  &  & 16 & 28 & 40 & 57 \\
 &  &  &  &  &  &  \\ \hline
\textbf{2} & \multicolumn{6}{c}{\textbf{Multi-task learning}} \\ \hline
2.1 & T1, T2 & T1, T2 & 18 & 45 & - & -  \\
2.2 & T1, T2, T3 & T1, T2, T3 & 18 & 32 & 21 & - \\
2.3 & T1, T2, T3, T4 & T1, T2, T3, T4 & 16 & 34 & 21 & 55 \\
 &  &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
\textbf{3} & \multicolumn{6}{c}{\textbf{Multi-task learning, addition of new task}} \\ \hline
3.1 & T1, T2 & T1, T2 (+ T3) & 18+16 & 45+34 & 21 & - \\
3.2 & T1, T2 & T1, T2 (+ T3, T4) & 18+16 & 45+34 & 22 & 49 \\
3.3 & T1, T2, T3 & T1, T2, T3 (+T4) & 18+12 & 32+34 & 21+21 & 46 \\ \hline
\textbf{4} & \multicolumn{6}{c}{\textbf{Multi-task learning, addition of new task with 50\% less training data}} \\ \hline
4.1 & T1, T2 & T1, T2 (+ T3) & 18+29 & 45+19 & 39 &  \\
4.2 & T1, T2 & T1, T2 (+ T3, T4) & 18+29 & 45+64 & 64 & 119 \\
4.3 & T1, T2, T3 & T1, T2, T3 (+T4) & 18+22 & 32+77 & 21+26 & 124 \\ \hline
\textbf{5} & \multicolumn{6}{c}{\textbf{Meta multi-task learning, meta testing phase involves addition of new task}} \\ \hline
5.1 & T1, T2 & T1, T2 (+ T3) & 282+1 & 496+5 & 21 & - \\
5.2 & T1, T2 & T1, T2 (+ T3, T4) & 282+3 & 496+1 & 3 & 16 \\
5.3 & T1, T2, T3 & T1, T2, T3 (+T4) & 356+1 & 354+15 & 356+4 & 16 \\
5.4 & T1, T2, T3, T4 & T1, T2, T3, T4 & 228 & 228 & 184 & 180 \\ \hline
\textbf{6} & \multicolumn{6}{c}{\textbf{Meta multi-task learning, meta testing phase involves addition of new task; with 50\% training data of new task}} \\ \hline
6.1 & T1, T2 & T1, T2 (+ T3) & 282 & 496+7 & 1 & - \\
6.2 & T1, T2 & T1, T2 (+ T3, T4) & 282+9 & 496+5 & 3 & 12 \\
6.3 & T1, T2, T3 & T1, T2, T3 (+T4) & 356+12 & 354+0 & 356+8 & 12 \\ \hline
\textbf{7} & \multicolumn{6}{c}{\textbf{Multi-task learning, leave one task out format}} \\ \hline
7.1 & T2, T3, T4 & T2, T3, T4 & - & 32 & 21 & 52 \\
7.2 & T1, T3, T4 & T1, T3, T4 & 16 & - & 21 & 51 \\
7.3 & T1, T2, T4 & T1, T2, T4 & 16 & 34 & - & 49 \\
7.4 & T1, T2, T3 & T1, T2, T3 & 18 & 32 & 21 & - \\ \hline
\textbf{8} & \multicolumn{6}{c}{\textbf{Multi-task learning, leave one task out format, addition of the left out task}} \\ \hline
8.1 & T2, T3, T4 & T2, T3, T4 (+ T1) & 10 & 32+34 & 21+25 & 52+26 \\
8.2 & T1, T3, T4 & T1, T3, T4 (+T2) & 16+17 & 24 & 21+15 & 51+20 \\
8.3 & T1, T2, T4 & T1, T2, T4 (+T3) & 16+17 & 34+34 & 9 & 49+26 \\
8.4 & T1, T2, T3 & T1, T2, T3 (+T4) & 18+8 & 32+34 & 21+21 & 9 \\ \hline
\textbf{9} & \multicolumn{6}{c}{\textbf{Meta multi-task learning, leave one task out format, addition of left out task in meta testing}} \\ \hline
9.1 & T2, T3, T4 & T2, T3, T4 (+ T1) & 4 & 359+6 & 361 & 360+9 \\
9.2 & T1, T3, T4 & T1, T3, T4 (+T2) & 48+12 & 21 & 226+18 & 226+9 \\
9.3 & T1, T2, T4 & T1, T2, T4 (+T3) & 306+1 & 304+25 & 232+4 & 304+23 \\
9.4 & T1, T2, T3 & T1, T2, T3 (+T4) & 356+1 & 354+15 & 356+4 & 16 \\ \hline
\end{tabular}%
}
\end{table*}
